Accelerating CNN inference on long vector architectures via co-design

CPU-based inference can be an alternative to off-chip accelerators, and vector architectures are a promising option due to their efficiency. However, the large design space of convolutional algorithms and hardware implementations makes it challenging to select the best options. This paper presents ongoing research into co-designing vector architectures for CPU-based CNN inference, focusing on the im2col+GEMM and Winograd kernels. Using the Gem5 simulator, we examine the impact of various hardware microarchitectural features on RISC-V Vector and ARM-SVE ISAs. We also study the impact of several BLIS-like algorithmic optimizations on im2col+GEMM. Our co-design study shows that longer vector lengths and larger caches can improve performance by 5x with our optimized CNN kernels, compared to a vector length of 512-bit and 1MB of L2 cache. For Winograd, we present a novel approach of inter-tile parallelization that exploits longer vector lengths and offers high memory reuse, resulting in up to 2.4x performance improvement for non-strided convolutional layers with 3x3 kernel size. Our study also shows that Winograd requires smaller cache sizes compared to im2col+GEMM.

==> areapower.tex <==

\sonia{ \color{blue} Our study proposes efficient optimizations on the software side as per the micro-architectural design and tuning of vector architectures as longer vector lengths at least up to 8192-bit with longer caches up to 256MB and 8 vector lanes to achieve maximum performance from vector processors. However, all these micro-architectural parameters tuning will have their impact on die-area and power consumption. This section focuses on the practicality of the recommended hardware parameters by extrapolating the area and power impact by keeping A64FX peak power consumption and area as the baseline.A64fx consumes a total power of 122 Watt ~\cite{yamamuraareapowera64fx} while running DGEMM, out of which $\sim$50\% i.e. $\sim$60 Watt is consumed by register files and vector unit. In the case of a pure SIMD vector processor, we expect the power and area consumed by the register file and vector unit will increases exponentially by increasing the SIMD width. With our assumptions, we extrapolate the power consumption and note the total power consumption for 1024-bit and 2048-bit SIMD processors as 182 Watt and 300 Watt respectively. If we keep increasing the SIMD width to 4K then power consumption will be a total of 540 Watt, which is very high power consumption. This will be a constraint in keep increasing the SIMD width beyond an extent. On the other hand in the case of pipelined vector processors, increasing the vector width only impacts the power consumption and area of the register file. In this way, we extrapolate the total consumption as 144 Watt for 1024-bit, 188 Watt for 2048-bit, 276 Watt for 4096-bit, and 454 Watt for 8192-bit. Similarly, the area of the die will get impacted on SIMD processors and pipelined vector processors. We can say that our design specifications contribute to assessing the relevant tradeoffs.   }

==> multicore.tex <==
\textit{OpenMP parallel for} pragmas are used for parallelizing the 6-Loops implementation of the GEMM kernel in the Darknet framework. From the Figure~\ref{fig:6loops}, OpenMP pragmas are used on the packing of the matrices (line 5, line 7) and on the top of macro-kernel at the line number 8.  Result~\ref{fig:YOLOV3-A64fx} presents the performance scalability with the optimized kernels on multiple cores using OpenMP on an A64FX machine.With scaling across the multi-core, our implementation achieves around 3.3$\times$ speedup. 

We have also checked the throughput achieved with the YOLOv3 network model by utilizing all system resources. The maximum throughput achieved is $\sim$1.2 seconds per frame i.e., $\sim$1 frame per second with the YOLOv3 bigger network model. With YOLOV3-Tiny performance scales upto 12 cores and throughput is 0.12 seconds per frame i.e. $\sim$10FPS . 

After analyzing the results statistics with increasing cores, "kmp-wait" is the main bottleneck with the increasing OpenMP threads. With statistics using the perf analysis tool, we have figured out that this is implicit barrier between the threads. 

\begin{figure}[ht!]
  \centering
  \includegraphics[width=.8\linewidth]{A64fx-scalability.pdf}
  \caption{YOLOV3 on A64FX}
%  \Description{YoloV3 on A64FX}
  \label{fig:YOLOV3-A64fx}
\end{figure}

We collected perf statistics using perf record after optimizing the kernels of convolutional layer on a single core.We observed that 81\% of time is consumed by setting up the network model. Rest 19\% is consumed by the prediction (computation part). Out of this 19\%, 14.5\% time is consumed by the GEMM kernel. %By the Amdhal's law speedup is limited by the fraction which can not be parallelized. 

%\begin{eqnarray}
%{Speedup} & <=\frac{1}{1-F}\\
%     & <= \frac{1}{1-0.76}\\
%     & <= 4
%\end{eqnarray}
%Where F is the fraction that is parallelizable. In our case 76\% is the fraction so upper bound of the speedup will be 4$\times$. 
In this respect, even if we expect the maximum achieved scalability by 4$\times$, the throughput will be $\sim$1 second per frame with YOLOv3 network.




==> parallel_performance_A64FX.tex <==

\subsection{Parallel performance on A64FX}
We investigate the multithreaded performance of our optimized 6-loop implementation of GEMM in Darknet on A64FX, which hosts 48 cores. We parallelize the kernel using OpenMP. In particular, we parallelize the loops in the packing of matrices and the macro-kernel (lines 5, 7 and 8 in  Fig.~\ref{fig:6loops}). Fig.~\ref{fig:YOLOV3-A64fx} demonstrates the speedup of YOLOv3 and YOLOv3-Tiny on 2 up to 48 cores, normalized to single core performance on A64FX, comparing our im2col+GEMM implementation against ARMPL. Our implementation achieves a speedup of 3.3$\times$ for YOLOv3, exceeding the speedup achieved by ARMPL, and a speedup of 2$\times$ for YOLOv3-Tiny. The maximum throughput achieved is 1.2 seconds per frame, i.e. $\sim$1 FPS for YOLOv3 on 48 cores, and 0.12 seconds per frame, i.e. $\sim$10 FPS, for YOLOv3-Tiny on 12 cores. 

A deeper analysis reveals that, in the case of YOLOv3 on 48 cores, 81\% of the execution time is consumed by the network initialization and only 19\% is corresponds to the computation part. Out of this 19\%, the parallel GEMM kernel consumes 14.5\% of the execution time. Therefore, the maximum attainable speedup is $\sim4\times$, in which case the maximum attainable throughput would be ~1 second per frame. 
%Additional profiling shows that, the main bottleneck in our parallel implementation is the implicit OpenMP barrier at the end of parallel for loops. 


%A deeper analysis with \texttt{perf} shows that the main bottleneck with the increasing number of threads in our parallel implementation is the implicit OpenMP barrier at the end of parallel for loops. 

%From the Figure~\ref{fig:6loops}, OpenMP pragmas are used on the packing of the matrices (line 5, line 7) and on the top of macro-kernel at the line number 8.  Result~\ref{fig:YOLOV3-A64fx} presents the performance scalability with the optimized kernels on multiple cores using OpenMP on an A64FX machine.With scaling across the multi-core, our implementation achieves around 3.3$\times$ speedup. 

%We have also checked the throughput achieved with the YOLOv3 network model by utilizing all system resources. The maximum throughput achieved is $\sim$1.2 seconds per frame i.e., $\sim$1 frame per second with the YOLOv3 bigger network model. With YOLOV3-Tiny performance scales upto 12 cores and throughput is 0.12 seconds per frame i.e. $\sim$10FPS . 

%After analyzing the results statistics with increasing cores, "kmp-wait" is the main bottleneck with the increasing OpenMP threads. With statistics using the perf analysis tool, we have figured out that this is implicit barrier between the threads. 

\begin{figure}[ht]
  \centering
  \includegraphics[width=.7\linewidth]{figs/A64fx-scalability.pdf}
  \caption{YOLOv3 speedup normalized to the single core on A64FX}
%  \Description{YoloV3 on A64FX}
  \label{fig:YOLOV3-A64fx}
  \vspace{-1.5em}
\end{figure}

==> programmability.tex <==
This section discusses the programmability comparison between ARM-SVE and RISC-V Vector. While doing the manual vectorizations with many algorithms, our study recommends the following improvements for RISC-V Vector programmability. 
The first is to have pointers with vector data types to give the flexibility to pass the vector data in the functions by their reference(call-by-reference) to have more readability and clean programming in the applications. 
The second is to provide the intrinsic instructions to transpose vector data and  instructions to merge/accumulate multiple vector type data. 

==> relatedwork.tex <==
The usage of CPUs for convolutional neural networks is not new. Several works focus on optimizations of CNNs on CPUs and evaluate inference performance~\cite{optimizingcnnoncpu, MLonfacebook, RuiliAnalyticalOpt}. However, the arrival of vector extensions spurred a new interest in academia and industry in optimizing different applications for these extensions and in assessing the impact of hardware parameters. Ramirez et al.~\cite{gem5benchmark} provide a new benchmark suite for RISC-V Vector and evaluate the impact the vector length and number of vector lanes, on applications from different domains. In the context of ARM-SVE, Poenaru et al.~\cite{processcachestudy} explore the effect of multiple micro-architectural parameters, such as vector lengths, L1/L2 cache line size, and associativity, on different HPC applications. Kodama et al.~\cite{ARMSVEAnalysisVL} evaluate common application kernels with different vector lengths and different numbers of physical registers using ARM-SVE. \nikela{We note that existing works do not evaluate the impact of the L2 cache size, which is an essential component in tuning the performance of new vector architectures, and an integral part of our work. Additionally, to the best of our knowledge, there is no existing work quantifying the impact of hardware parameters in the context of CNN inference, using optimized kernels for vector architectures.  }
%Additionally, existing work does not quantifies the impact of micro-architectural parameters with optimized kernels in the context of CNN inference.


The new vector extensions for CPUs have driven optimizations in a multitude of neural network frameworks. Louis et al. ~\cite{tensorlite} port and optimize convolutional and matrix multiplication kernels of CNNs in TensorFlow Lite on RISC-V Vector, achieving a reduction of instructions. %This paper has studied only the number of reduced instructions but has not presented the performance analysis. 
Iliescu et al.~\cite{gemmarm-sve} optimize the General Matrix Multiplication (GEMM) and low precision GEMM kernels on ARM-SVE, using loop unrolling and vectorization. 
%This paper presents the algorithmic optimizations with loop unrolling with vectorization and does not focus on blis-like optimizations. 
CPU vendors have also optimized neural network frameworks to leverage the ARM-SVE vector extensions. Fujitsu provides an optimized version of the OneDNN Deep Neural Network library~\cite{intelonednn}, using just-in-time compilation techniques to generate high-performance code for ARMv8 with SVE from x86 functions. Additionally, ARM provides optimized CNN kernels using ARM-SVE in the ARM Compute Library \cite{ARMComputeLibrary}, focusing on the im2col+GEMM. \nikela{Our work offers highly optimized CNN kernels for both RISC-V Vector and ARM-SVE vector extensions, by jointly examining the effect of multiple algorithmic optimizations on vector architectures with different micro-architectural parameters. Beyond the commonly used im2col+GEMM kernel, we additionally contribute the first optimized version of convolutional layers using the Winograd algorithm, in a vector-length-agnostic way, on ARM-SVE. }
%In the context of ARM-SVE, To achieve high DNN performance, Fujitsu has optimized the OneDNN Deep Neural Network library~\cite{intelonednn} for the ARM-SVE architecture using just-in-time compilation techniques to generate high-performance code for ARMv8 with SVE from x86 functions. 
%Iliescu et al.~\cite{gemmarm-sve} described optimizations to General Matrix Multiplication (gemm) and low precision gemm computational kernels. This paper presents the algorithmic optimizations with loop unrolling with vectorization and does not focus on blis-like optimizations. 
%Arm has optimized the CNN kernels in ARM Compute Library[13] and mainly focuses on the im2col + gemm approach. 



%sonia{All these studies of optimizations miss an opportunity to study the co-designing of the algorithmic optimizations on different vector architectures with awareness of their micro-architecture's design. Our paper shows that not all optimizations are relevant to all types of vector architectures. On RISC-V Vector, where the vector processor is attached to the L2 cache and there is no prefetcher, we show that BLIS-like optimizations do not improve performance. 
%The previous work does not study the Winograd implementation for the convolutional layers with longer vectors on VLA architectures. Our paper contributes the very first optimized implementation of a convolutional layer with 3x3 kernel size using Winograd in a vector length agnostic way, showcasing the performance improvement on real hardware/simulation environment for inference where network models include CNN layers with 3x3 kernel sizes. }

